SeaFormer++: Squeeze-enhanced Axial Transformer for Mobile Visual Recognition

Since the introduction of Vision Transformers, the landscape of many computer vision tasks (e.g., semantic segmentation), which has been overwhelmingly dominated by CNNs, recently has significantly revolutionized. However, the computational cost and memory requirement renders these methods unsuitable on the mobile device. In this paper, we introduce a new method squeeze-enhanced Axial Transformer (SeaFormer) for mobile visual recognition. Specifically, we design a generic attention block characterized by the formulation of squeeze Axial and detail enhancement. It can be further used to create a family of backbone architectures with superior cost-effectiveness. Coupled with a light segmentation head, we achieve the best trade-off between segmentation accuracy and latency on the ARM-based mobile devices on the ADE20K, Cityscapes, Pascal Context and COCO-Stuff datasets. Critically, we beat both the mobilefriendly rivals and Transformer-based counterparts with better performance and lower latency without bells and whistles. Furthermore, we incorporate a feature upsampling-based multi-resolution distillation technique, further reducing the inference latency of the proposed framework. Beyond semantic segmentation, we further apply the proposed SeaFormer architecture to image classification and object detection problems, demonstrating the potential of serving as a versatile mobile-friendly backbone. Our code and models are made publicly available at https://github.com/fudan-zvg/SeaFormer.

==> algorithm/algorithm.tex <==
\begin{figure}[tp]
\begin{minipage}[c]{0.48\textwidth}
%   \vspace{0pt}  
    

\end{minipage}%
\hspace{0.5em}
\begin{minipage}[b]{0.5\textwidth}
  \vspace{0pt}
  
\end{minipage}
% \label{alg: nr soft}
\end{figure}

==> algorithm/newton_raphson.tex <==
\begin{algorithm}
\SetAlgoLined
\KwIn{$A\in \mathbb{R}^{m\times m}$, and $\mathcal{T}\in \mathbb{Z}^+$}{$\alpha= 2/\|A\|_1^2$.Initialize $A_0\leftarrow \alpha A$}\;
\For{$k$ from $1$ to $\mathcal{T}$ }{
$A_{k}\leftarrow 2A_{k-1}-A_{k-1}AA_{k-1}$
}
\KwOut{$A_\mathcal{T}$}
 \caption{NR: Newton-Raphson iteration}
 \label{NR}
\end{algorithm}

==> algorithm/soft.tex <==
\begin{algorithm}
\SetAlgoLined
\KwIn{$Q\in \mathbb{R}^{n\times d_e}$, sampling function $f_s$}
\KwSty{Sampling}  $\ \widetilde{Q} \leftarrow f_s(Q)$ \;
$A\leftarrow\text{exp}(\widetilde{Q}\ominus \widetilde{Q})$, $P\leftarrow\text{exp}(\widetilde{Q}\ominus Q)$\;
$\hat{S}\leftarrow P^\top \text{NR}(A) P$\;
\KwOut{$\hat{S}$}
 \caption{SOFT: Softmax-free attention}
 \label{soft}
\end{algorithm}

==> table/rebuttal_coco.tex <==
\begin{table}[tb]
    \centering
    \small
    \begin{tabular}[b]{l | c |c |c }
    \hline

    \hline

    \hline
        Backbone & AP  & FLOPs    & Params\\
    \hline
        
    \hline
    \hline
    AxialFormer~\cite{wang2020axial} & 37.7  & 210G  & 23.7M  \\
    SeaFormer-L &  39.8      & 185G  &24.0M            \\
    \textbf{SeaFormer-L++} &  \textbf{40.2}       & \textbf{185G}    &24.1M            \\
         \hline

        \hline
        
        \hline
  \end{tabular}
\caption{\textcolor{blue}{Results on COCO object detection.}}
\label{table_coco_obj_2}
\end{table}

==> table/rebuttal_imagenet.tex <==
\begin{table*}
% \vspace{-1.1cm}
\small
\centering

\begin{tabular}{L{4.0cm}|C{1.5cm}|C{1.5cm}|C{1.5cm}|C{1.5cm}}
\hline

\hline

\hline
Method  & Params  &FLOPs & Top1 & Latency\\
\hline

\hline
\hline
AxialFormer~\cite{wang2020axial} & 11.6M & 3.0G & 78.1 & 151ms\\
SeaFormer-L & 14.0M & 1.2G & 79.9 & 61ms \\ 
\textbf{SeaFormer-L++} & 14.1M & 1.2G & \textbf{80.6} & \textbf{61}ms \\ 
\hline

\hline

\hline
\end{tabular}
\caption{\textcolor{blue}{Image classification results on ImageNet-1K \textit{val} set. The FLOPs and latency are measured with input size 224×224, except for MobileViT and MobileViTv2 that are measured with 256×256 according to their original implementations. * indicates re-parameterized variants~\cite{vasu2022improved}. The latency is measured on a single Qualcomm Snapdragon 865, and only an ARM CPU core is used for speed testing. No other means of acceleration, e.g., GPU or quantification, is used.}}
\label{imagenet_table_3}
% \vspace{-2.2cm}
\end{table*}
